LLM-Oriented Retrieval Tuner

Dense Retrieval (DR) is now considered as a promising tool to enhance the memorization capacity of Large Language Models (LLM) such as GPT3 and GPT-4 by incorporating external memories. However, due to the paradigm discrepancy between text generation of LLM and DR, it is still an open challenge to integrate the retrieval and generation tasks in a shared LLM. In this paper, we propose an efficient LLM-Oriented Retrieval Tuner, namely LMORT, which decouples DR capacity from base LLM and non-invasively coordinates the optimally aligned and uniform layers of the LLM towards a unified DR space, achieving an efficient and effective DR without tuning the LLM itself. The extensive experiments on six BEIR datasets show that our approach could achieve competitive zero-shot retrieval performance compared to a range of strong DR models while maintaining the generation ability of LLM.

==> Tables/Tab.multi-lmort.tex <==
\begin{wraptable}{l}{6.5cm}
\vspace{-2.2em}
\caption{The NDCG@10 results of multiple LMORT plugins mounted on a GPT-j-6B. $\mathbf{L}$ means the layer number of LMORT. \label{tab:multi-lmort}}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
%% ************************************
\multirow{2}{*}{\textbf{Datasets}} & \multicolumn{4}{c}{\textbf{LMORT (NDCG@10)}} & \multirow{2}{*}{\textbf{Best L}} \\
& \textbf{$\mathbf{L}$=1} & \textbf{$\mathbf{L}$=2} & \textbf{$\mathbf{L}$=3} & \textbf{$\mathbf{L}$=4} & \\
\hline
COVID & 0.598 & 0.719 & \textbf{0.735} & 0.718 & \textbf{2} \\
NFCorpus & 0.273 & 0.283 & 0.280 & \textbf{0.296} & \textbf{4} \\
FiQA &  0.206 & 0.243 & \textbf{0.251} & 0.247 & \textbf{3} \\
ArguAna & \textbf{0.499} & 0.487 & 0.476 & 0.451 & \textbf{1} \\
SciFact & 0.657 & 0.659 & \textbf{0.679} & 0.666 & \textbf{3} \\
SCIDOCS & 0.125 & \textbf{0.128} & 0.126 & 0.124 & \textbf{2} \\
\bottomrule
\end{tabular}}
\end{wraptable}


% COVID & 0.718 \\
% NFCorpus & 0.296 \\
% FiQA & 0.247 \\
% ArguAna & 0.451 \\
% SciFact & 0.666 \\
% SCIDOCS & 0.124 \\



